Snapshot Difference Imaging using Time-of-Flight Sensors

Computational photography encompasses a diversity of imaging techniques, but one of the core operations performed by many of them is to compute image differences. An intuitive approach to computing such differences is to capture several images sequentially and then process them jointly. Usually, this approach leads to artifacts when recording dynamic scenes. In this paper, we introduce a snapshot difference imaging approach that is directly implemented in the sensor hardware of emerging time-of-flight cameras. With a variety of examples, we demonstrate that the proposed snapshot difference imaging technique is useful for direct-global illumination separation, for direct imaging of spatial and temporal image gradients, for direct depth edge imaging, and more.

==> related.tex <==
\section{Related work}\label{sec:related}

Sensor technology: Lock-in pixels (PMDs) \cite{lange1999time}, multi-bucket pixels \cite{wan2012cmos}. Cite Dorrington lock-in paper

Skellam noise in difference imaging \cite{hwang2012difference}

Applications: 

Gradient cameras: spatial \cite{tumblin2005gradient}, temporal contrast sensor \cite{lichtsteiner2008temporalcontrast}

Direct-global separation: \cite{nayar2006fast}\cite{otoole2012primal}(better: cite Matt's CVPR 2014 paper which has the camera relayed over DMD) \cite{HeideOE2014,Wu2012}

Detecting skin \cite{anderson1981optics,jones2002statistical}


